Dissertation Paths: Advisors and Students in the Economics Research Production Function

Elite economics PhD programs aim to train graduate students for a lifetime of academic research. This paper asks how advising affects graduate students' post-PhD research productivity. Advising is highly concentrated: at the eight highly-selective schools in our study, a minority of advisors do most of the advising work. We quantify advisor attributes such as an advisor's own research output and aspects of the advising relationship like coauthoring and research field affinity that might contribute to student research success. Students advised by research-active, prolific advisors tend to publish more, while coauthoring has no effect. Student-advisor research affinity also predicts student success. But a school-level aggregate production function provides much weaker evidence of causal effects, suggesting that successful advisors attract students likely to succeed-without necessarily boosting their students' chances of success. Evidence for causal effects is strongest for a measure of advisors' own research output. Aggregate student research output appears to scale linearly with graduate student enrollment, with no evidence of negative class-size effects. An analysis of gender differences in research output shows male and female graduate students to be equally productive in the first few years post-PhD, but female productivity peaks sooner than male productivity.

==> Exhibits/tables/Freq_DI.tex <==
Accounting Review&1985&2123\\
Aea Papers And Proceedings&2018&776\\
American Economic Journal: Applied Economics&2009&628\\
American Economic Journal: Economic Policy&2009&678\\
American Economic Journal: Macroeconomics&2009&540\\
American Economic Journal: Microeconomics&2009&654\\
American Economic Review&1985&7099\\
American Economic Review: Insights&2019&154\\
American Journal Of Agricultural Economics&1985&4441\\
American Political Science Review&1985&1679\\
Annals Of The AAPSS&1998&1955\\
Annual Review Of Financial Economics&2009&74\\
Brookings Papers On Economic Activity&1985&1380\\
Canadian Journal Of Economics&1985&2375\\
Carnegie-Rochester Conference Series On Public Policy&1985&410\\
Columbia Journal Of World Business&1994&99\\
Contemporary Accounting Research/Recherche Comptable Contemporaine&2003&1189\\
Demography&1985&2241\\
Econometric Theory&1990&1474\\
Econometrica&1985&2488\\
Economic Development And Cultural Change&1985&1318\\
Economic Inquiry&1985&2587\\
Economic Journal&1985&3432\\
Economic Record&1985&1335\\
Economic Theory&1991&2611\\
Economica&1985&1389\\
Economics Letters&1988&11136\\
European Economic Review&1985&4262\\
European Journal Of Operational Research&2015&4274\\
Experimental Economics&1998&719\\
Explorations In Economic History&1985&945\\
Financial Analysts Journal&2012&299\\
Financial Management&1990&1020\\
Games And Economic Behavior&1989&3396\\
Ilr Review&2015&361\\
Industrial And Labor Relations Review&1985&1102\\
Industrial Relations&1985&1098\\
Informs Journal On Applied Analytics&2017&178\\
Interfaces&2012&212\\
International Economic Review&1985&2079\\
International Journal Of Production Economics&1994&7052\\
International Monetary Fund Staff Papers&1985&437\\
International Organization&1985&971\\
Journal Of Accounting And Economics&1985&1176\\
Journal Of Accounting Research&1985&1372\\
Journal Of Banking And Finance&1985&5743\\
Journal Of Business&1985&700\\
Journal Of Business And Economic Statistics&1985&2134\\
Journal Of Business Ethics&2020&1104\\
Journal Of Business Finance And Accounting&2005&957\\
Journal Of Consumer Affairs&1986&1003\\
Journal Of Consumer Research&1985&2133\\
Journal Of Corporate Finance&1994&2262\\
Journal Of Development Economics&1985&3059\\
Journal Of Econometrics&1985&4414\\
Journal Of Economic And Social Measurement&1985&536\\
Journal Of Economic Behavior And Organization&1985&5799\\
Journal Of Economic Dynamics And Control&1985&3816\\
Journal Of Economic Education&1985&1430\\
Journal Of Economic History&1985&1390\\
Journal Of Economic Literature&1985&822\\
Journal Of Economic Perspectives&1987&1918\\
Journal Of Economic Theory&1985&4008\\
Journal Of Economics And Business&1985&1182\\
Journal Of Economics And Management Strategy&1992&1032\\
Journal Of Environmental Economics And Management&1985&2141\\
Journal Of Finance&1985&3093\\
Journal Of Financial And Quantitative Analysis&1985&1915\\
Journal Of Financial Economics&1985&3271\\
Journal Of Financial Intermediation&1990&708\\
Journal Of Financial Markets&1998&665\\
Journal Of Financial Research&1985&1054\\
Journal Of Financial Services Research&1987&866\\
Journal Of Futures Markets&1985&1928\\
Journal Of Health Economics&1985&2303\\
Journal Of Human Resources&1985&1465\\
Journal Of Industrial Economics&1985&1109\\
Journal Of International Business Studies&1998&1484\\
Journal Of International Economics&1985&2448\\
Journal Of International Money And Finance&1985&2879\\
Journal Of Labor Economics&1985&1274\\
Journal Of Law And Economics&1985&1083\\
Journal Of Law Economics And Organization&1985&934\\
Journal Of Legal Studies&1988&780\\
Journal Of Marketing Research&2009&975\\
Journal Of Mathematical Economics&1985&2226\\
Journal Of Monetary Economics&1985&2690\\
Journal Of Money Credit And Banking&1985&2649\\
Journal Of Peace Research&1993&1323\\
Journal Of Political Economy&1985&2097\\
Journal Of Portfolio Management&1985&2013\\
Journal Of Public Economics&1985&3829\\
Journal Of Risk And Insurance&1985&1375\\
Journal Of Risk And Uncertainty&1988&912\\
Journal Of The American Statistical Association&1985&4118\\
Journal Of The European Economic Association&2003&1240\\
Journal Of The Royal Statistical Society: Series A &1985&24\\
Journal Of The Royal Statistical Society: Series A (Statistics In Society)&1988&1366\\
Journal Of The Royal Statistical Society: Series B (Statistical Methodology)&2016&410\\
Journal Of Urban Economics&1985&1926\\
Kyklos&1985&1009\\
Land Economics&1985&1551\\
Management Science&2012&1999\\
Manufacturing And Service Operations Management&2009&563\\
Marketing Science&1985&1621\\
Mathematical Finance&1995&814\\
Mathematical Methods Of Operations Research&1995&1165\\
Monthly Labor Review&1985&2279\\
NBER Macroeconomics Annual&1986&553\\
National Tax Journal&1985&1685\\
Operations Research&2009&1263\\
Oxford Economic Papers&1985&1495\\
Oxford Economic Papers N. S.&1986&214\\
Population And Development Review&1985&1329\\
Proceedings Of The National Academy Of Sciences&1996&393\\
Production And Operations Management&2014&1421\\
Public Choice&1985&3586\\
Quantitative Economics&2010&391\\
Quarterly Journal Of Economics&1985&1715\\
Quarterly Journal Of Political Science&2006&287\\
Quarterly Review Of Economics And Business&1985&219\\
Rand Journal Of Economics&1985&1523\\
Research Policy&1997&3196\\
Review Of Accounting Studies&1996&890\\
Review Of Economic Dynamics&1998&1161\\
Review Of Economic Studies&1985&1922\\
Review Of Economics And Statistics&1985&3108\\
Review Of Finance&2004&780\\
Review Of Financial Studies&1989&2376\\
Scandinavian Journal Of Economics&1985&1648\\
Social Choice And Welfare&1985&2086\\
Social Science Quarterly&1985&2832\\
Southern Economic Journal&1985&2533\\
Transportation Research: Part B: Methodological&1999&2310\\
Urban Affairs Review&2005&770\\
World Development&1985&6841\\


==> Exhibits/tables/Freq_Top6.tex <==
\begin{tabular}{lcc}
\toprule
\multicolumn{3}{c}{Top-6} \\
\midrule
Journal & First Year Indexed & Papers \\
\midrule
Aea Papers And Proceedings&2018&776\\
American Economic Review&1985&7099\\
Econometrica&1985&2488\\
Journal Of Political Economy&1985&2097\\
Quarterly Journal Of Economics&1985&1715\\
Review Of Economic Studies&1985&1922\\
Review Of Economics And Statistics&1985&3108\\
\bottomrule
\end{tabular}


==> Exhibits/tables/Gender_Networks.tex <==
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi} \begin{tabular}{lcccccccc} \hline \hline
& \multicolumn{4}{c}{Levels} & \multicolumn{4}{c}{Poisson} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
&\multicolumn{2}{c}{DI}&\multicolumn{2}{c}{T6}&\multicolumn{2}{c}{DI}&\multicolumn{2}{c}{T6} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
&\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\ 
\hline
Female dummy    &    -0.40\sym{***}&    -0.39\sym{***}&    -0.11\sym{***}&    -0.11\sym{***}&    -0.28\sym{***}&    -0.27\sym{***}&    -0.34\sym{***}&    -0.33\sym{***}\\
                &  (0.068)         &  (0.068)         &  (0.025)         &  (0.026)         &  (0.049)         &  (0.049)         &  (0.081)         &  (0.083)         \\
[1em]
Female share by cohort and school&                  &    -0.14         &                  &   -0.051         &                  &    -0.11         &                  &    -0.26         \\
                &                  &   (0.43)         &                  &   (0.18)         &                  &   (0.28)         &                  &   (0.49)         \\
\hline
Dep. var. mean  &     1.54         &                  &     0.36         &                  &     1.54         &                  &     0.36         &                  \\
R2              &    0.044         &    0.044         &    0.042         &    0.042         &                  &                  &                  &                  \\
\hline\hline  \end{tabular}


==> Exhibits/tables/Table2.tex <==
\begin{tabular}{lccccccccc}
\toprule
& \multicolumn{3}{c}{Economics} & \multicolumn{3}{c}{Related} & \multicolumn{3}{c}{Other} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
& Total & Cohort size & Active & Total & Cohort size & Active & Total & Cohort size & Active \\
& (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) \\ 
\toprule
\\ \multicolumn{8}{l}{Panel A. 1989-2023 Graduates} \\\\ [-1ex]
Berkeley&1119&32.0&&158&4.5&&344&9.8&\\
Chicago&897&25.6&&155&4.4&&276&7.9&\\
Harvard&1139&32.5&&169&4.8&&406&11.6&\\
MIT&865&24.7&&217&6.2&&71&2.0&\\
Northwestern&675&19.3&&75&2.1&&82&2.3&\\
Princeton&650&18.6&&39&1.1&&117&3.3&\\
Stanford&759&21.7&&325&9.3&&258&7.4&\\
Yale&660&18.9&&101&2.9&&83&2.4&\\
All&6764&24.2&&1239&4.4&&1637&5.8&\\
\\ \multicolumn{8}{l}{Panel B. 1994-2017 Graduates} \\\\ [-1ex]
Berkeley&854&35.6&.46&103&4.3&.36&244&10.2&.09\\
Chicago&681&28.4&.38&105&4.4&.53&148&6.2&.17\\
Harvard&791&33.0&.54&91&3.8&.42&281&11.7&.31\\
MIT&631&26.3&.58&150&6.3&.31&42&1.8&.07\\
Northwestern&485&20.2&.54&54&2.3&.50&60&2.5&.17\\
Princeton&467&19.5&.57&27&1.1&.44&75&3.1&.2\\
Stanford&530&22.1&.48&216&9.0&.46&156&6.5&.19\\
Yale&454&18.9&.52&52&2.2&.29&48&2.0&.17\\
All&4893&25.5&.50&798&4.2&.41&1054&5.5&.19\\
\bottomrule
\end{tabular}


==> Exhibits/tables/Table6_3yearsgrouped_all_vs_3endogenous_t6.tex <==
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi} \begin{tabular}{lcccccccc} \hline \hline
& \multicolumn{4}{c}{All features instrumented} & \multicolumn{4}{c}{First 3 instrumented} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} 
&\multicolumn{2}{c}{DI}&\multicolumn{2}{c}{T6}&\multicolumn{2}{c}{DI}&\multicolumn{2}{c}{T6} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
&\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\ 
\hline
Advisor Research&     0.16\sym{*}  &     0.17\sym{**} &    0.042         &    0.044         &     0.18\sym{**} &     0.18\sym{**} &    0.065\sym{*}  &    0.065\sym{*}  \\
                &  (0.090)         &  (0.086)         &  (0.042)         &  (0.041)         &  (0.085)         &  (0.084)         &  (0.039)         &  (0.038)         \\
[1em]
Advising Load   &   -0.018         &   -0.019         &   -0.010         &   -0.010         &   -0.026         &   -0.027         &   -0.015         &   -0.015         \\
                &  (0.027)         &  (0.024)         &  (0.012)         &  (0.012)         &  (0.026)         &  (0.025)         &  (0.011)         &  (0.011)         \\
[1em]
Past Student Success&     0.11         &    0.041         &    0.085         &    0.073         &     0.12         &    0.084         &    0.095         &    0.084         \\
                &   (0.21)         &   (0.22)         &  (0.080)         &  (0.084)         &   (0.20)         &   (0.20)         &  (0.076)         &  (0.076)         \\
[1em]
Coauthored with Advisor Pre-grad&   -0.017         &    -0.37         &     0.99         &     0.92         &   -0.056         &    -0.10         &     0.25         &     0.23         \\
                &   (2.17)         &   (2.18)         &   (0.92)         &   (0.93)         &   (0.24)         &   (0.23)         &   (0.15)         &   (0.15)         \\
[1em]
Coauthored with Classmate Pre-grad&                  &    -0.48         &                  &     0.16         &                  &     0.75\sym{*}  &                  &     0.27         \\
                &                  &   (3.11)         &                  &   (1.43)         &                  &   (0.43)         &                  &   (0.26)         \\
[1em]
Any Publication Pre-grad&     1.37         &     1.37         &     0.43         &     0.40         &     1.74\sym{***}&     1.65\sym{***}&     0.46\sym{***}&     0.43\sym{***}\\
                &   (1.21)         &   (1.27)         &   (0.50)         &   (0.52)         &   (0.15)         &   (0.15)         &  (0.068)         &  (0.071)         \\
[1em]
Cites Advisor in Thesis&                  &     1.02         &                  &     0.14         &                  &     0.31\sym{***}&                  &    0.091\sym{**} \\
                &                  &   (0.64)         &                  &   (0.27)         &                  &  (0.084)         &                  &  (0.036)         \\
\hline
Dep. var. mean  &     1.56         &                  &     0.39         &                  &     1.56         &                  &     0.39         &                  \\
\hline\hline  \end{tabular}


==> Exhibits/tables/rolling_super_duper_turbo_std_DI_stdpro_econ_related_2024_T6.tex <==
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi} \begin{tabular}{lcccccccc} \hline \hline
& \multicolumn{4}{c}{Levels} & \multicolumn{4}{c}{Poisson} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} 
&\multicolumn{2}{c}{DI}&\multicolumn{2}{c}{T6}&\multicolumn{2}{c}{DI}&\multicolumn{2}{c}{T6} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
&\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\ 
\hline
Advisor Research&     0.15\sym{***}&                  &    0.087\sym{***}&                  &    0.084\sym{***}&                  &     0.15\sym{***}&                  \\
                &  (0.023)         &                  &  (0.011)         &                  &  (0.012)         &                  &  (0.018)         &                  \\
[1em]
Advising Load   &  0.00016         &                  &  0.00069         &                  &   0.0027         &                  &   0.0053         &                  \\
                & (0.0073)         &                  & (0.0030)         &                  & (0.0046)         &                  & (0.0068)         &                  \\
[1em]
Past Student Success&     0.33\sym{***}&                  &    0.095\sym{***}&                  &     0.20\sym{***}&                  &     0.27\sym{***}&                  \\
                &  (0.041)         &                  &  (0.017)         &                  &  (0.022)         &                  &  (0.035)         &                  \\
[1em]
Super Advisor Research&                  &     0.28\sym{***}&                  &     0.14\sym{***}&                  &     0.17\sym{***}&                  &     0.34\sym{***}\\
                &                  &  (0.062)         &                  &  (0.028)         &                  &  (0.035)         &                  &  (0.058)         \\
[1em]
Super Advising Load&                  &     0.13         &                  &    0.040         &                  &     0.13\sym{*}  &                  &     0.31\sym{**} \\
                &                  &  (0.090)         &                  &  (0.037)         &                  &  (0.068)         &                  &   (0.14)         \\
[1em]
Super Past Student Success&                  &     0.29\sym{***}&                  &    0.073\sym{**} &                  &     0.20\sym{***}&                  &     0.23\sym{***}\\
                &                  &  (0.075)         &                  &  (0.033)         &                  &  (0.046)         &                  &  (0.081)         \\
[1em]
Duper Advisor Research&                  &     0.28\sym{***}&                  &     0.18\sym{***}&                  &     0.16\sym{***}&                  &     0.35\sym{***}\\
                &                  &  (0.047)         &                  &  (0.022)         &                  &  (0.025)         &                  &  (0.038)         \\
[1em]
Duper Advising Load&                  &     0.30\sym{***}&                  &     0.10\sym{***}&                  &     0.24\sym{***}&                  &     0.46\sym{***}\\
                &                  &  (0.085)         &                  &  (0.035)         &                  &  (0.064)         &                  &   (0.14)         \\
[1em]
Duper Past Student Success&                  &     0.63\sym{***}&                  &     0.19\sym{***}&                  &     0.37\sym{***}&                  &     0.45\sym{***}\\
                &                  &  (0.098)         &                  &  (0.041)         &                  &  (0.053)         &                  &  (0.091)         \\
\hline
Dep. var. mean  &     1.56         &                  &     0.39         &                  &     1.56         &                  &     0.39         &                  \\
R2              &    0.082         &    0.076         &    0.084         &    0.081         &                  &                  &                  &                  \\
\hline\hline  \end{tabular}

